Label Leakage and Protection in Two-party Split Learning

Two-party split learning is a popular technique for learning a model across feature-partitioned data. In this work, we explore whether it is possible for one party to steal the private label information from the other party during split training, and whether there are methods that can protect against such attacks. Specifically, we first formulate a realistic threat model and propose a privacy loss metric to quantify label leakage in split learning. We then show that there exist two simple yet effective methods within the threat model that can allow one party to accurately recover private ground-truth labels owned by the other party. To combat these attacks, we propose several random perturbation techniques, including $\texttt{Marvell}$, an approach that strategically finds the structure of the noise perturbation by minimizing the amount of label leakage (measured through our quantification metric) of a worst-case adversary. We empirically demonstrate the effectiveness of our protection techniques against the identified attacks, and show that $\texttt{Marvell}$ in particular has improved privacy-utility tradeoffs relative to baseline approaches.

==> tex/max_norm_alignment.tex <==
% \subsubsection{Max norm alignment to prevent label leakage}
% \label{sec:max_norm_alignment}

We now introduce an improved way to add Gaussian noise by making the expected norm of the positive and negative gradients in a mini-batch equal (un-distinguishable). The key question is how to determine the standard deviation of the Gaussian noise with zero mean added to each gradient. For simplicity, we can align all the instances to have the same expected norm with the maximum gradient norm among the mini-batch. Hence, we name this heuristic protection method as {\tt max\_norm}. %It's worth mentioning that the instance which has the maximum norm is a positive one. 
Suppose that instance $i$ in a mini-batch has the maximum gradient norm and its corresponding gradient is $g_i$. For arbitrary $j$,
let instance $j$'s gradient be $g_j$. 
The noise we add is $\eta_j\cdot g_j$, where $\eta_j\sim \mathcal{N}(0,\sigma_j^2)$ and $\sigma_j$ is the standard deviation to be determined. 
The perturbed gradient of $g_j$ is $g'_j = g_j(1+\eta_j)$,
and we require (the square of) the expected norm of ${g'_j}^2$ to be aligned to that of $g_i$,
% The standard deviation $\sigma_j$ of the Gaussian noise added to perturbate the gradient $g_j$ is calculated by making their expected norm equal, 
then we have: $$\|g_i\|_2^2=\mathbb{E}(||g_j||^2(1 + \eta_j)^2) =  ||g_j||^2(1 + \sigma_j^2).$$ Hence $\sigma_j = \sqrt{{||g_i||^2}/{||g_j||^2} - 1}$. As designed, \maxnorm \ can prevent the norm attack very well (more details can be seen in the experimental section). The advantage of \maxnorm \ is that it has no parameter to tune. Unfortunately, it does not have a theoretical guarantee of the trade-off between model utility and privacy and it may be breached by some unknown attacks. 

% \begin{equation}
% \begin{split}
% E(||g_i||^2) = E(||g_j||^2(1 + 2 \sigma_j + \sigma_j^2)) \\
% E(||g_i||^2) = E(||g_j||^2(1 + \sigma_j^2)) \\
% \sigma_j^2 = \frac{||g_i||^2}{||g_j||^2} - 1   \\
% \sigma_j = \sqrt{\frac{||g_i||^2}{||g_j||^2} - 1} \\
% \end{split}
% \end{equation}

% The corresponding algorithm is described as Algorithm~\ref{alg:max_norm}.

% \begin{algorithm}[H]
% \DontPrintSemicolon
%   \KwInput{$\mathbf{g}$: gradient sending back to the passive party; $n$ by $d$ where $n$ is the batch size, $d$ is the number embedding dimension. \;}
%   \KwOutput{$\mathbf{g'}$: perturbated gradient with Gaussian noise}
%     compute $max\_norm$ =  max($||\mathbf{g}_i||^2$),  $\forall i \in [1, n]$ \\
%  \For{i \leftarrow 1 \ to \ n}    
%         { \tcc{compute the standard deviation of the Gaussian noise}
%         $\sigma_i = \sqrt{max(\frac{||max\_norm||^2}{||\mathbf{g}_i^2||} - 1, 0)}$ \\
%         $noise_i \sim \mathcal{N}(0,\,\sigma_i^{2})$ \tcp*{generate the zero mean Gaussian noise}\\
%         $\mathbf{g'}_i = \mathbf{g}_i (1 + noise_i)$ \tcp*{add the generated noise to the gradient} \\
%         }
%  \textbf{Return} $\mathbf{g'}$
% \caption{Max Norm Alignment to Preventing Label Leakage}
% \label{alg:max_norm}
% \end{algorithm}

% The disadvantage of this algorithm is that it does not have a theoretical guarantee.
